Critical Reflections on Visualization Authoring Systems

An emerging generation of visualization authoring systems support expressive information visualization without textual programming. As they vary in their visualization models, system architectures, and user interfaces, it is challenging to directly compare these systems using traditional evaluative methods. Recognizing the value of contextualizing our decisions in the broader design space, we present critical reflections on three systems we developed -- Lyra, Data Illustrator, and Charticulator. This paper surfaces knowledge that would have been daunting within the constituent papers of these three systems. We compare and contrast their (previously unmentioned) limitations and trade-offs between expressivity and learnability. We also reflect on common assumptions that we made during the development of our systems, thereby informing future research directions in visualization authoring systems.

==> sections/04b-selection.tex <==
% !TEX root =  ../main.tex
%% =======================================================================
\subsection{Selection}
%% =======================================================================

Selecting appropriate visualization components is a prerequisite for performing direct manipulation and data binding operations. The level of selection support depends on the component abstractions exposed by each of the three systems. 

In Lyra, marks are the primary target for selection, and authors can resize and rotate marks through handles. \leo{How does selecting anchor points work in Lyra? Also, when I was playing with Lyra, there was some container that I could select. How did it work exactly?} 

Data Illustrator exposes a set of hierarchically organized components: at the lowest level, anchor points and line/curve segments are the graphical primitives to describe paths. Marks include not only path-based shapes (e.g. rectangles and ellipses), but also texts and images. Multiple marks are then organized into groups or collections, which can be nested. The selection mechanism follows this hierarchy. Clicking once selects the top level collection, double clicking opens up the collection so that the individual marks can be selected. \leo{Is it necessary to include a figure?} This design closely follows the selection model in Adobe XD. The selection of anchor points and segments follows the interaction paradigm used in Adobe Illustrator, where a different tool (direct selection) is used. 

Charticulator provides a similar set of hierarchical visualization components: anchors and handles, marks, glyphs (which correspond to groups in Data Illustrator \leo{Is this true?}), and plot segments (which correspond to collections in DI \leo{Is this true?}). Charticulator provides two separate editing canvases: a glyph editor, and a chart canvas. \leo{Is it necessary to include a figure?} The selection of marks and anchor points can thus take place in either the glyph editor or the chart canvas. Selecting a glyph or a plot segment solely happens in the chart canvas. 

To emulate existing design applications, all three systems also support selecting marks, glyphs/groups, and collections in a layers panel.

The differences between selectable components and selection mechanisms between the three systems stem from both the visualization model and interface design choices. Since Lyra maps interactions to declarative statements in the Vega visualization grammar, which does not formally represent graphical primitives such as line segments, there are fewer types of selectable components. Data Illustrator and Charticulator, on the other hand, consider data binding to be constraints on vector graphics, thus provide a richer set of selectable components. The design of selection model in Data Illustrator resembles the models in Adobe XD and Adobe Illustrator, so that authors familiar with these systems will not need any training. Selecting a mark can be tedious, however, if authors intend to select a mark embedded in multi-level nested collections - multiple double clicks are needed to open up the collections hierarchically. To avoid this problem and reduce visual clutter, Charticulator provides a separate editing canvas for glyphs and enables more flexible and easier selection. 


% - All: list of items in a panel (conformity w/graphics systems, select layers/items)
%   - Layering? Lyra, Charticulator yes. DI (not implemented).
% - Charticulator: glyph, plot segment from the canvas; mark from the glyph editor; anchor points from both
% - DI: hierarchical (collection of shapes > one shape > normal, direct selection)
% - Lyra: marks + anchor points




==> sections/dirty-secrets.tex <==
% !TEX root =  ../main.tex
%% =======================================================================
\section{Discussion: The ``Dirty Little Secrets'' of Expressivity}
%% =======================================================================

\todo{Intro paragraph. Parallel structure to assumptions section: author, system, data.}

% From John's email: dirty.tex
The previous section explored ways in which our three systems differ in their approach to the tradeoff of expressivity versus
learnability. In this section, we discuss similarities and shared characteristics of the systems, focusing on aspects where a person
approaching them may be caught off-guard or may have expectations of capabilities they do not provide. Again, we divide the discussion into aspects pertaining to data, author, and system.

%Data
%% =================================
\subsection{Data and Transformations}
%% =================================
5
In Section 3.1 we explained how all three systems assume that some level of data cleaning and transformation is performed outside the
tool before visualization construction. This assumption may seem straightforward, but it has implications toward the visualization
creation process.

Consider the slope chart infographic example from the front cover of Alberto Cairo's book {\em The functional art}\cite{Cairo2012Functional}. This graphic
represents a dataset containing the percentage of college educated and obese residents, respectively, in the 50 U.S. states. Each data
category is mapped along a vertical axes, with higher values moving up each axis. A state thus is represented as a line with its two
endpoints at the corresponding value positions on the two axes. All 50 states' lines are shown in the graph.  Cairo chose to color lines with a positive slope (left axis value lower than right axis value) red and lines with a negative slope blue.

Imagine designing this visualization in one of our systems. In all likelihood, the dataset would contain one row for each state with two
columns per row, for the obesity and college rate percentages respectively. How would a designer specify the color of each line from
this data set?  The relative simplicity of the data and the objective suggests that this should be easily accomplished in the
system. However, the logic dictating line color is really a derived value, requiring a mathematical operation on the two values for a
state.

To create this visualization in one of our systems, the designer would likely derive a new third column using a spreadsheet, one containing the sign (e.g., 1 or -1) of the slope of the line. Creating a new column this way is not an overly onerous burden, but it illustrates how creating a visualization from an original dataset may reuire further transformational intervention. This makes sense if one considers the broad scope of visualizations -- frequently, marks or characteristics of marks in the view represent dervied aspects of data, maybe simple mathmatical transformations at the simplest or complex models of the data in a more complex scenario.


%commenting out the old text
%Although supporting a rich set of data wrangling capabilities~\cite{kandel2011wrangler} is out of scope, how these systems should narrow schematic congruency remains an open question. As Lyra illustrates, it is not sufficient to simply extend the underlying visualization models to provide data transformation capabilities as expecting users to invoke and define them manually still presents a non-trivial semantic distance. Instead these systems must develop higher-level scaffolding that automatically infers or suggests appropriate transformations when necessary (analogous to their existing mechanisms for data binding which automatically infer definitions for scales and guides).

%- Charticulator + DI: no data transformation facilities (except for sorting? Summary stats?)
%- Lyra: rich palette of transformations.
%  - But instantiated via property inspectors. Not really direct manipulation. 
%- Full data wrangling out of scope, but inherently part of design. 
%  - Leaky abstraction: e.g., deriving/calculating new fields require specifying formulas. Is this programming?
%- Alberto Cairo’s slope chart.




%% =================================
\subsection{Accessibility}
%% =================================

Motor impairments, color blindness

%% =================================
\subsection{Alternate Modalities}
%% =================================

E.g., non mouse/touch screen.



==> sections/improvement.tex <==
\section{Areas for Improvement in the Systems}

The previous section explored ways in which our three systems both
differ and share similarities in their approach to the tradeoff of
expressivity versus learnability. In this section, we discuss more of
the commonalities of the three systems, focusing on 
areas or aspects in which they currently may not provide capabilities
that one would expect or desire, effectively areas with room for
improvement.

%===================================================
\subsection{Data Manipulation and Transformation}
%===================================================

In Section ~\autoref{sec:assumptions} we explained how all three systems assume that some
level of data cleaning and transformation is performed outside the
tool before visualization construction. This assumption may seem
straightforward, but it has implications toward the visualization
creation process.

Consider the slope chart infographic example from the front cover of
Alberto Cairo's book \todo{{\em The functional art}\cite{Cairo2012Functional}}. This graphic
represents a dataset containing the percentage of college educated and
obese residents, respectively, in the 50 U.S. states. Each data
category is mapped along a vertical axes, with higher values moving up
each axis. A state thus is represented as a line with its two
endpoints at the corresponding value positions on the two axes. All 50
states' lines are shown in the graph.  Cairo chose to color lines with
a positive slope (left axis value lower than right axis value) red and
lines with a negative slope blue.

Imagine designing this visualization in one of our systems. In all
likelihood, the dataset would contain one row for each state with two
columns per row, for the obesity and college rate percentages,
respectively. How would a designer specify the color of each line from
this data set? The relative simplicity of the data and the objective
suggests that this should be easily accomplished in the
system. However, the logic dictating line color is really a derived
value, requiring a mathematical operation on the two values for a
state.

To create this visualization in one of our systems, the designer would
likely derive a new third column using a spreadsheet, one containing
the sign (e.g., 1 or -1) of the slope of the line. Creating a new
column this way is not an overly onerous burden, but it illustrates
how creating a visualization from an original dataset may require
further transformational intervention. This makes sense if one
considers the broad scope of visualizations---frequently, marks or
characteristics of marks in the view represent derived aspects of
data, maybe simple mathematical transformations at the simplest or
complex models of the data in a more complex scenario.

\john{Now go into a little discussion about how this is really ``visual
programming'' that we want, the long history of that area, and how
it's really difficult to do in a general sense. There could even be a
little discussion about how our systems really are forms of visual
programming systems for this specific domain (visualization design)
and we should explore ideas from the visual programming community to
make our tools even more powerful and capable.}


%===================================================
\subsection{Support Design, not Only Construction}
%===================================================

\john{Here we discuss how the systems currently work relatively well for
someone who begins with a design in mind, and then simply wants to
build it. However, the systems do not function as well for people who
just bring their data with no representation in mind, and they want to
explore different design ideas and possibilities. The tools need to
provide better assistance for ideation and sketching to develop
initial design ideas.}


%===================================================
\subsection{Adaptability Across Different Datasets}
%===================================================

Currently, the systems are primarily constructed to work with a specific
dataset and design a visualization for it. However, users may
subsequently bring a different data set, still with the same
``structure,'' that is, the same columns and types of values in each
column, and want their design to also work for it.

\john{To be honest, I am not sure how well the systems do this now. It is my
impression from what I recall that Charticulator (especially) and Lyra
(somewhat) can partially do this now a bit better than Data
Illustrator can. However, even with that said, it's also my
impression that it would be easy to bring another data set where the
values are just ``right'' so that the visual binding initially
constructed effectively breaks, that is, it just doesn't look right.
Ideally, we would want our initial designs with a dataset to be
flexible and generalizable so that they adapt intelligently to
different datasets that may have slightly different characteristics
(e.g., more extreme values, etc.)}

\bongshin{It depends on what you mean by ``different.'' Charticulator can reuse the chart design with other datasets (i.e., with differnt values) but having the same structure (i.e., same data types at the very least; it might be the case that it has to have the same column name.}
\bongshin{Additional (important) aspect is to handle imperfect datasets depending on semantics.}


%===================================================
\subsection{Multiple ``Views'' in a Visualization}
%===================================================

\john{This one I'm unsure about. Sometimes a designer wants to create a
visualization that effectively has subregions in the window/view, each
containing a different fundamental representation of the data. Thus, a
particular data item and its attributes may have multiple
representations in a view.  I don not believe that the systems can
currently support this at a most fundamental level. I guess it would
be possible to just design the different subviews independently and
somehow stitch them together using the underlying language/library,
but one might want something deeper than that.  This also connects to
the last subsection below in terms of brushing and linking then.}

\bongshin{Charticulator's framework is designed with this in mind---this is partly why we have a Plot Segment element/component. Donghao showed one example during his talk at VIS last year---scatterplot and bar chart connected by links, if I remember correctly. I believe that it was implemented after the submission.}


%===================================================
\subsection{Animation and Interaction}
%===================================================

All three systems are primarily designed to create static
visualizations and infographics.  \john{(Again here, I believe that may not
be true for Lyra because of the underlying Vega capabilities,
etc. Please clarify that as needed.)}

It would be terrific if the systems also allowed users to create
animated visuals. For instance, a dataset may be time series data and
the designer wants to show how values change and evolve over time.

Finally, it would be great if the systems also could generate
interactive visualizations. This could likely range from relatively
simple interactions (e.g., tooltip presentation of data values on
mouse-over) to much more rich and complex interactive behaviors,
perhaps even with control widgets. If a visualization does support
subviews (item above), then the construction tools could support
brushing and linking.




==> sections/old-conclusion.tex <==
% !TEX root =  ../main.tex
%% =======================================================================
\section{Conclusion}
%% =======================================================================

In this paper, we contribute critical reflections on three visualization authoring systems\,---\,Lyra~\cite{satyanarayan2014lyra}, Data Illustrator~\cite{liu2018data}, and Charticulator~\cite{ren2019charticulator}\,---\,which were all designed and developed to increase expressivity in visualization design via interactive interfaces.
Through a series of in-depth discussions, we extracted the similarities and differences in their approaches and how they were a result of trading off expressivity for learnability, or vice-versa. Reflecting on the commonalities in the assumptions (or scopes) we had, we identified opportunities to advance the design of interactive visualization authoring systems.

%Looking ahead, we see two core future research directions for expressivity and learnability.
%For the former, extending the systems to support animated or interactive visualization would be the next logical step for increasing expressivity.
%Currently, even relatively simple animations (e.g., updating bar heights) or interactions (e.g., tooltips or brushing and linking) can require non-trivial programming or textual specification. 
%How might authoring systems support such visualizations while maintaining their interactive and direct manipulation affordances? 
%Are there limits to such approaches\,---\,for instance, could they be used to author complex animations such as the ``bar chart race''~\cite{Burn-Murdoch2019bar}?


% As all three systems are primarily designed to create static
% visualizations and infographics, a logical next step is to further increase expressivity by supporting animated or interactive visualizations.
% Both of these could range from relatively simple to rich and complex.
% For instance, designers may want to show how values change evolve over time with a simple animated line chart. It would be also great to enable people to create an exciting, more complex animation such as ``bar chart race'' without programming. 
%https://observablehq.com/@johnburnmurdoch/bar-chart-race
% The interaction could range from a simple tooltip presentation on mouse-over to brushing and linking between multiple views within a chart.
%much more rich and complex interactive behaviors, perhaps even with control widgets. If a visualization does support subviews (item above), then the construction tools could support .

%Moreover, highly flexible, interactive systems typically require meaningful tutorials to onboard novice users. For example, our systems all provide video recordings of creating example visualizations, which authors can follow to learn system functionality. Charticulator takes this idea a step further by augmenting the video play with content segmentation and textual descriptions. However, as systems evolve, it becomes increasingly expensive keep such videos up-to-date. As Ren et al. describe~\cite{ren2018reflecting}, we see great potential and need for interactive tutorials that can co-evolve with the systems themselves.

%- Different modalities
%- Interaction
%- Animation
%- Interactive Tutorials 

This paper provides a new type of contribution to the visualization community~\cite{lee2019contribution}: a constructive set of ``lessons learned'' synthesized from critical reflections on the development and public deployment of complex interactive systems.
We note that, even for the creators of one of the three systems, it would have been infeasible to attain these details and insights by merely studying the other two systems and their corresponding publications.
The visualization research community could benefit from more in-depth and critical reflections on systems developed with a similar goal, making collaborative progress.

==> xarchive/00-abstract.tex <==
\abstract{An emerging generation of visualization authoring systems support expressive information visualization without textual programming. As they vary in their visualization models, system architectures, and user interfaces, it is challenging to directly compare these tools using traditional evaluative methods. Recognizing the value of contextualizing our decisions in the broader design space, we present critical reflections on three systems we developed\,---\,Lyra, Data Illustrator, and Charticulator.
This paper surfaces knowledge that would have been daunting within the constituent papers of these three systems.
We compare and contrast their (previously unmentioned) pitfalls, limitations, and trade-offs between three design dimensions: expressivity, learnability, and reusability.
We also describe how the process of critical reflection shapes our ongoing research agenda and informs future research directions in visualization authoring systems.}

% Arvind
% Bongshin
% Donghao
% Jeff
% John S
% John T
% Matt
% Z Leo 


%There is a growing demand among analysts, designers, and other practitioners to visualize data in highly expressive ways without writing code. To address this need, a new generation of visualization authoring tools has emerged over the past few years. These tools claim to support expressive information visualization while requiring no programming expertise. An objective evaluation and comparison of these tools is difficult, however, as they vary greatly in terms of their visualization models, system architectures, and user interfaces. This paper brings together the authors of Lyra, Data Illustrator, and Charticulator to critically reflect on the expressivity, learnability, and reusability of these visualization systems. Through these candid reflections, we share knowledge that would not usually be included in a typical system research paper: the rationales and tradeoffs between design dimensions, the pitfalls and limitations of the systems, and the opportunities for future research.

%We--the creators of Lyra, Data Illustrator, and Charticulator--present critical reflections on the design and development of this new generation of visualization authoring systems along the dimensions of expressivity, learnability, and reusability. In response to a growing demand among analysts, designers, and other practitioners to visualize data in highly expressive ways without writing code, our main goal with these systems was to support expressive information visualization while requiring no programming expertise. However, because they vary greatly in their visualization models, system architectures, and user interfaces, it is challenging to directly compare these tools based on traditional objective measures. We instead share knowledge that would not usually be included in a typical system research paper--the rationales and justifications of design decisions, the tradeoffs and tensions between design considerations, as well as the (unmentioned) pitfalls and limitations of the systems.



%The new generation of visualization authoring tools share a common goal\,---\,maximizing the set of visualizations that can be constructed without textual specification\,---\,but vary in terms of their visualization models, system architectures, and user interfaces. In recognition that it can be difficult for any one system to fully contextualize its decisions in the broader system design space, we present critical reflections on three systems\,---\,Lyra, Data Illustrator, and Charticulator\,---\,exploring tensions and trade-offs along three design dimensions: expressivity, learnability, and reusability. Our goal is to surface knowledge that would not be usually included in a typical system research paper or a comparative evaluation paper - the rationales and justifications of design decisions, the (unmentioned) pitfalls and limitations of the systems



% ARVIND VERSION
%\arvind{The new generation of visualization authoring tools share a common goal\,---\,maximizing the set of visualizations that can be constructed without textual specification\,---\,but vary in terms of their visualization models, system architectures, and user interfaces. In recognition that it can be difficult for any one system to fully contextualize its decisions in the broader system design space, we present critical reflections on three systems\,---\,Lyra, Data Illustrator, and Charticulator\,---\,exploring tensions and trade-offs along three design dimensions: expressivity, learnability, and reusability.}

% ARVIND'S VERSION BASED ON LEO'S
%\arvind{A new generation of visualization authoring tools, which support expressive information visualization without textual programming, has emerged. As they vary in their visualization models, system architectures, and user interfaces, it is challenging to directly compare these tools using traditional evaluative methods. Recognizing the value of contextualizing our decisions in the broader design space, we present critical reflections on three systems we developed\,---\,Lyra, Data Illustrator, and Charticulator.
%We surface knowledge that would have been difficult for any individual paper to do so\,---\,comparing and contrasting their complexities, how they navigated trade-offs and tensions between design considerations, as well as the (unmentioned) pitfalls and limitations of the systems.}

% the trade-offs and tensions between expressivity, learnability, efficiency, and reusability

% compares and contrasts the complexities of these systems, the assumptions that we made during their respective development process, and the resulting shortcomings of these systems,

%%MATT VERSION
%\matt{We present a critical reflection of Lyra, Data Illustrator, and Charticulator, integrating the perspectives of their respective creators and focusing on the themes of expressivity, learnability, and reusability. These three systems are members of a new class of visualization authoring environments that strive to maximize a set of design choices via an interactive interface. However, this expressivity is provided at the cost of complexity, though this complexity manifests differently across our three systems. Of interest to prospective and fellow system developers in the visualization community, our candid discussion compares and contrasts the complexities of these systems, the assumptions that we made during their respective development process, and the resulting shortcomings of these systems, a discussion that was largely absent in the Lyra, Data Illustrator, and Charticulator papers.}

%%LEO VERSION
%\leo{A new generation of visualization authoring tools has emerged over the past few years, claiming to support expressive information visualization without writing code. Since they vary greatly in their visualization models, system architectures, and user interfaces, it is challenging to directly compare these tools based on traditional measures in controlled studies. In this paper, we – the creators of Lyra, Data Illustrator, and Charticulator – present critical reflections on the design and development of these three systems. Our goal is to surface knowledge that would not be usually included in a typical system research paper or a comparative evaluation paper - the rationales and justifications of design decisions, the (unmentioned) pitfalls and limitations of the systems, and the tradeoffs and tensions between design considerations along three dimensions: expressivity, learnability and reusability.}


%% DONGHAO VERSION
% \donghao{Recently there is a new generation of visualization authoring tools that share a common goal --- maximizing the set of visualizations that can be constructed without textual programming. In response to the trade-offs between expressivity, learnability, efficiency, and reusability, they vary in terms of their visualization models, system architectures, and user interfaces. In this paper we --- the creators of Lyra, Data Illustrator, and Charticulator --- present critical evaluations of these systems. We share constructive knowledge that are not typically included in a systems research paper --- 
% the design rationales, the tradeoffs, and tensions between design considerations, as well as the (unmentioned) pitfalls and limitations of the systems.}


==> xarchive/01-introduction.tex <==
%% The ``\maketitle'' command must be the first command after the
%% ``\begin{document}'' command. It prepares and prints the title block.

%% the only exception to this rule is the \firstsection command
%% ==============================
\firstsection{Introduction}
%% ==============================

\maketitle

An increasing number of interactive systems enable people to visually communicate information with charts~\cite{rost2016,kirk2019}.
However, the expressive range of any single system is often limited to predefined chart templates, each with a small number of configurable parameters.
In contrast, the most expressive ways to visualize data involve the use of either vector design tools such as Adobe Illustrator or powerful yet low-level libraries such as D3.js~\cite{bostock2011d3} or declarative grammars such as Vega~\cite{satyanarayan2016reactive}.
%Both approaches can be used in conjunction with advanced vector graphics illustration software to fine-tune the output~\cite{Bigelow2017Hanpuku}. 
However, producing highly custom charts remains out of reach for most people, being considerably time-consuming or requiring programming expertise.
In response, a new generation of interactive visualization authoring systems has emerged aiming to bridge the gap between the rigidity of template-based approaches and the often impractical freedom of programmatic approaches.

As the creators of three systems belonging to this new generation\,---\,Lyra~\cite{satyanarayan2014lyra}, Data Illustrator~\cite{liu2018data}, and Charticulator~\cite{ren2019charticulator}, we are uniquely poised to comment upon their common goal of increasing expressivity in visualization design via interactive interfaces.
While these systems have a shared motivation, they are notably different in terms of their underlying frameworks, system architectures, and interface designs.
As these systems differ along these main aspects, it can be not only challenging but also undesirable or even nonsensical to perform a controlled comparative evaluation between a new system and its predecessors~\cite{ren2018reflecting}.
The differences are confounds that can be difficult to quantify, and thus any results are likely to be misleading and biased in favor of the new system. 
Instead, it is more valuable to the visualization research community and to fellow system developers that we contextualize our decisions in the broader design space. We set out to provide a balanced and deep examination on the respective approaches and capabilities of visualization authoring systems through \textit{critical reflection}.

The key contributions of this paper are twofold.
First, we critically reflect on the design of Lyra, Data Illustrator, and Charticulator, going beyond what we respectively knew when wrote the constituent papers that introduced these three systems, focusing specifically on the aspects of expressivity, learnability, and reusability.
Second, we discuss how the process of critical reflection shapes our ongoing research agenda and informs future research directions in visualization authoring systems.
We hope that this paper can serve as an example of providing a different type of contribution to the visualization community: a constructive set of lessons learned through critical reflection on the development of complex interactive systems.

% We provide critical reflections of the three visualization authoring systems we have developed in terms of expressivity, learnability, and reusability.
%We discuss how the series of discussions reflecting on the design and development of these systems influenced our research agenda regarding interactive visualization authoring systems, as well as future research directions to further advance this new generation of visualization authoring systems.

% Lyra: 2014; Data Illustrator & Charticulator: 2018
% We are witnessing the rise of data-driven storytelling~\cite{riche2018data,stolper2018,segel2010narrative}: people are in need of creating custom and expressive charts going beyond conventional ones to better convey core messages and engage the audience.
% The most powerful and flexible way of creating a novel chart is to program it using a library (e.g., D3.js~\cite{bostock2011d3}) or a declarative language (e.g., Vega~\cite{satyanarayan2016reactive}).
% However, this approach requires programming expertise and thus is not accessible to many of practitioners including designers and journalists.
% %In his inspiring talk at the Stanford HCI seminar, Victor presented a tool for creating visualizations via direct manipulation~\cite{victor2013}. 
% This prompted the emergence of a new generation of visualization authoring tools such as iVisDesigner~\cite{ren2014ivisdesigner}, Lyra~\cite{satyanarayan2014lyra}, Data Illustrator~\cite{liu2018data}, and Charticulator~\cite{ren2019charticulator}, which do not require programming.

% Although these tools share a similar high-level goal--achieve higher expressivity with graphical user interfaces--they are drastically different in terms of underlying framework and system architectures.
% However, expressivity is a complex notion and their main focus and approach are usually not the same as we researchers strive to devise new approaches.
% As such, it is challenging (or even undesirable) to perform a traditional comparative evaluation between these systems~\cite{ren2018reflecting}. 
%Still, to provide the evidence of the system's efficiency and usability, we resort to conventional lab studies and emphasize positive aspects of the system.
%In other words, we are losing an opportunity to share constructive and useful knowledge that could benefit the research community.








%- Democratization of visualization
%In industry, practitioners, people w/o expertise, graphic designers, etc.
%Vis seen as a necessary skill
%Not necessarily bringing programming knowledge to table
%- Different tools available: Tableau to Chart makers to D3
%- New generation of tools has emerged (Lyra, DI, Chartic)
%No “programming”, just show what it looks like, add data binding
%Seek to increase expressivity of designer
%	Expressivity can be a complex notion though
%- How does one compare, evaluate and assess these tools?
%Seem almost too good to be true. How far can they go? Where do they fail?
%- Good time to engage in an expert critique of them
%	System designers know pitfalls to avoid and dirty little secrets
%	Also know nuances of approach and rationale/justifications
%	Help research community understand +/- and suggest compelling opportunities for future work
%Can share constructive and useful knowledge not usually surfaced
%- Seek a more balanced and deep examination on approach, design, and capabilities of these systems

==> xarchive/02-background.tex <==
%% =====================================
\section{Background and Related Work}
%% =====================================

In this section we present an overview of visualization design and authoring, and briefly recapitulate the three visualization authoring systems --- Lyra~\cite{satyanarayan2014lyra}, Data Illustrator~\cite{liu2018data}, and Charticulator~\cite{ren2019charticulator} --- which form the subject of our critical reflection.
More importantly, we reflect on the implications of scoping our tools as visualization authoring systems.

\subsection{Approaches to Visualization Design}
TODO: A (brief) history of approaches to visualization design;
TODO: Modern visualization design and Meeks’ “Three Waves” categorization~\cite{Meeks2018}.
Bottom-up vs. Top-down paper \cite{mendez2017bottomup}
Mendez agency discussion \cite{mendez2018agency}
Huron paper on constructive visualization \cite{Huron2014Constructive}.

% In a survey of visualization construction user interfaces, Grammel \etal~\cite{Grammel2013Survey} defined ``visualization construction'' as the step from data tables to visual structures in Card \etal's visualization reference model~\cite{TODO:Card1999}. 
% - Terminology: design vs. authoring   (?)

\emph{Visualization design} is the general process of visualizing data. For the purpose of data analytics, visualization designs includes figuring out the domain problem, the dataset, the task, the visual representation, as well as the algorithms and computer programs for realizing the design~\cite{munzner2014visualization}.
For the purpose of communicative visualization, the design process includes generating findings from data, creating the visual representations, as well as annotating the visualizations and articulating them with supplemental material to clearly convey the findings.
Visualization design includes the exploration of design possibilities in an iterative process;  designers make decisions on visual encodings, data content, and the overall composition \cite{Bigelow2014DesignWithData}.

We consider \emph{visualization authoring} as a process within visualization design.
Authoring refers to the more narrow process of implementing an existing visualization design given a prepared dataset.
We assume that the author already has a desired visual representation in mind and the data in the appropriate form for said design.

\subsection{Visualization Authoring Tools}

\subsubsection{Imperative and Declarative Programming}


A wide variety of frameworks, libraries, and declarative languages for creating visualizations with textual programming or specification have been created.
Alternately, multiple widely adopted visualization programming toolkits and libraries such as Processing~\cite{Reas2006Processing}, D3~\cite{bostock2011d3}, and Vega~\cite{satyanarayan2016reactive} exist. While such toolkits and libraries achieve the ultimate expressivity, it requires considerable programming expertise to fully master them.
\emph{The Grammar of Graphics}~\cite{wilkinson1999grammar} forms the basis of many visualization grammars, including ggplot~\cite{Wickham2006ggplot} and Vega-Lite~\cite{Satyanarayan2017VegaLite}. Visualization grammars allows authors to use concise and uniform languages to represent a wide variety of visualizations.

% An \emph{interactive} visualization authoring system still include an underlying visualization framework or grammar. The choice of the underlying framework has a strong implication on the expressivity, learnability, and reusability of the visualization authoring system.

\subsubsection{Interactive Visualization Authoring Systems}

%% Situate our systems in the wide space of authoring tools. What makes these systems unique? What are common in these systems?

Grammel \etal~\cite{Grammel2013Survey} surveyed previous visualization construction user interfaces (aka., interactive visualization authoring tools or systems ). % this doesn't apply to the storytelling and communication aspect.
Many commercial products, such as Microsoft Excel, uses the \emph{template editor} approach. The expressivity of this approach is limited to the set of availiable templates. It is worth mentioning that some commercial products allows extensive customization of their templates (\eg by providing a variety of fonts, color schemes, and graphical styles).
% - Commercial products - template tools
\emph{Shelf construction} is adopted in analytic-oriented tools such as Tableau~\cite{TODO:tableau}. Instead of using predefined templates, these tools allow authors to map data fields to encoding channels (\eg x, y, color, width, height). The system is responsible for generating a proper visualization based on the author's specification.
- Drawing focused tools
- Constraint-based tools

\subsubsection{Summary of Our Three Systems}

This paper reflect on the design of three interactive visualization authoring systems: Lyra~\cite{satyanarayan2014lyra}, Data Illustrator~\cite{liu2018data}, and Charticulator~\cite{ren2019charticulator}. Here we briefly recapitulate the key aspects of these systems. For more details, we direct the reader to the original research papers and websites.

\bpstart{Lyra} \url{http://idl.cs.washington.edu/projects/lyra/}

\bpstart{Data Illustrator} \url{http://data-illustrator.com/}

\bpstart{Charticulator} \url{https://charticulator.com/}



\subsection{Evaluating Authoring Toolkits and Systems}
Dan Olsen paper~\cite{olsen2007} and similar   (?)
Ledo et al (CHI 2018)~\cite{Ledo2018}: Evaluation Strategies for HCI Toolkit Research
Recent meta-reflections  (Amini \& Brehmer - DDS~\cite{Amini2018DDS}, Ren et al - BELIV~\cite{ren2018reflecting})
Lam et al. 7 Scenarios~\cite{lam2012empirical}.

\subsection{Employing Critical Reflection as an Evaluation Method}





==> xarchive/03-reflections.tex <==
%% =====================================
\section{Critical Reflections of Three Systems}
%% =====================================

In their classic paper on the past, present, and future of user interface toolkits, Myers, Hudson, and Pausch~\cite{myers:past} describe such systems as having a ``ceiling'' and ``threshold''\,---\,how much can be done with the system, and how difficult it is to learn to use the system, respectively. They identify the inherent tension between these two properties, and note that most successful systems either have a low ceiling and low threshold or a high ceiling and a high threshold. In this section, we critically reflect on how, in balancing expressivity and learnability, this same tension manifests in interactive visualization authoring systems, and how it is further exacerbated by an additional concern: reusability.

\subsection{What These Systems Assume}

The three systems designed by the authors of this paper share several assumptions regarding the data they ingest, the people using the system, the working environment in which the system is used, and how the content produced with the system might be used. 

\bstart{The data}
With regards to the data that people load into these systems, the assumption is that the data is a tidy CSV or TSV file. Based on the example charts showcased in the systems' respective papers and online galleries, the size of the datasets in these files is also small: a handful or columns and dozens of rows, or a few hundred rows at most. There are no missing or erroneous values, and the data has already been appropriately cleaned, filtered, and aggregated using some other set of data analysis and preparation tools. Finally, the data is static, meaning that the structure or values of the data will not change at some later point in the design process.

\bstart{The author}
What do these systems assume about the author, the person using the system to create a custom chart? Above all, these systems assume that the author already has a chart design in mind. Perhaps it is something they sketched on paper, or maybe they want to emulate a design they saw elsewhere, such as in the system's associated online gallery. Second, they assume that the author and the data are already acquainted, that a process of exploratory data analysis and data preparation has already occurred. Beyond this, it is difficult to make assumptions about the authors, such as what other design and data analysis tools they use in the course of their work, their level of visualization literacy, or their industry and job title; perhaps they are a data scientist, a journalist, or a graphic designer. Lastly, these systems assume a single author working in isolation.

\bstart{The environment}
As with the author, these systems also make assumptions about the working environment in which they work. First, when we make video recordings of these systems or demonstrate them in public settings, we tend to use large high-resolution displays with a mouse. While this may reflect the working environments of many who try these tools, we anticipate that many will be using smaller laptop displays with a trackpad or a touchscreen, and the systems were not optimized for these device profiles. Second, all three of our systems are web-based and run in a web browser, presupposing that people will be willing and permitted to upload their data into a web browser. Both Lyra and Charticulator are open source systems, so it is conceivable that those concerned with keeping their data private could build and run these systems from their local machines, though this additional work may remain to be a barrier to adoption.

\bstart{The content}
Once that all of the aforementioned assumptions are met and that the author has used one of these systems to produce content, let us consider how this content be exported and (re)used. The systems are agnostic about the context in which this content will be used; these contexts might include live presentations, websites, or print articles. Irrespective of the context, one common export format between these systems is SVG (Scalable Vector Graphics), which will present well across a range of display sizes. SVG also allows authors to make further additions to the content in applications like Adobe Illustrator~\cite{Bigelow2017Hanpuku}. Regardless of the export format, the exported content from these systems is non-interactive. Both Lyra and Charticulator also anticipate other downstream uses of the content, expressing it as a Vega JSON specification~\cite{satyanarayan2016reactive} in the case of the former and as a JSON template or as a Power BI custom visual specification~\cite{PowerBI} in the case of the latter. In both cases, these systems are not producing chart instances but rather chart components that might be later populated with other data sharing the same schema.  

\input{sections/03a-expressivity.tex}
\input{sections/03b-learnability.tex}
\input{sections/03c-reusability.tex}

==> xarchive/03a-expressivity.tex <==
\subsection{Expressivity}

Lyra, Data Illustrator, and Charticulator all define ``expressivity'' in the same way: what is the gamut of visualizations that can be created with the system? This definition maps neatly to the earlier ``ceiling'' term, and is a natural one for these systems to adopt as they explore a new modality for authoring visualizations\,---\,direct manipulation. Yet, despite this common goal, the three systems make different choices on how to maximize their expressive ceilings, centering on how each system models visualization specification.

%Lyra maps user interactions to declarative statements in the Vega visualization grammar~\cite{satyanarayan2016reactive}. Users never explicitly specify any control flow but instead use drag and drop interactions to establish data joins, connect marks for relative positioning and labeling, and customize layout algorithms. Data Illustrator, on the other hand, couples two core operations\,---\,repeat and partition\,---\,with a ``lazy'' data bind. Finally, Charticulator poses visualization design as a constraint satisfaction problem, while leveraging drag and drop interactions. Users specify layout constraints, such as anchoring a shape to the minimum value or linking sibling marks together, which are solved by the system to produce the desired visualization.

%\leo{
Lyra maps user interactions to declarative statements in the Vega visualization grammar~\cite{satyanarayan2016reactive}. Visualizations are thus the output of compiling declarative grammars. Users never explicitly specify any control flow but instead use drag and drop interactions to establish data joins, connect marks for relative positioning and labeling, and customize layout algorithms. Data Illustrator and Charticulator both treat visualizations as vector graphics constrained by data binding, but differ in their emphases. 
Data Illustrator augments vector design tools with two core operations\,---\,repeat and partition\,---\, as well as ``lazy'' data bindings. Users draw paths, generate shapes by data and specify bindings between data variables and visual properties to constrain the behavior of free-form graphics. Charticulator, on the other hand, dives deeper to focus on layout as a constraint satisfaction problem, while leveraging drag and drop interactions. Users specify layout constraints, such as anchoring a shape to the minimum value or linking sibling marks together, which are solved by the system to produce the desired visualization.
%}

These differences in visualization models are informed by the chronology of development\,---\,Lyra is the oldest system, followed by Data Illustrator and then Charticulator, each responding to perceived limitations in the prior systems. Thus, it may be tempting to consider Charticulator's system of constraints to be the most expressive. But, if we adopt a broader definition of expressivity, we can engage in a deeper analysis that reveals a more nuanced set of strengths and limitations. In particular, Hutchins, Hollan, and Norman~\cite{hutchins:direct} break expressions in an interface language down into two components: \textbf{what} can be expressed, or the \emph{semantic distance}, and \textbf{how} is it expressed, or the \emph{articulatory distance}. Our previous definition of expressivity only covered the first of these two aspects, and although the second closely relates to our subsequent discussion of learnability, we consider these dimensions together here as a way to better contrast the tradeoffs each system made.

%======================================================
\subsubsection{Semantic Distance: What is Expressible?}
%======================================================
An interface's semantic distance refers how closely a user is able to map their intentions to its primitives\,---\,i.e., does an interface expose concepts and make distinctions in the same way the user thinks about them? \leo{The original paper \cite{hutchins:direct} characterizes semantic distance using two questions: ``Is it possible to say what one wants to say in this language? '', and ``Can the thing of interest be said concisely?''. Exposing concepts and making distinctions in the same way are related to the first question. Both questions seem to be about the gulf of execution.} Semantic distances occur on both the input and output sides of an interface. For instance, higher-level languages reduce the input semantic distance by allowing users to omit low-level details \leo{This seems to be a good example of ``Can the thing of interest be said concisely?''} whereas WYSIWYG (``What You See Is What You Get'') editors narrow the output semantic distance as the effect of editing commands can be seen instantly. \leo{To me this is more about the gulf of evaluation: providing feedback to uses so that they can assess if the goal has been achieved. This seems to be different from the two questions raised earlier. I understand that the original paper groups all these things under the term ``semantic distance'', which is much broader than just ``what is expressible''. Should we try to make a clearer distinction here?}

In this regard, all three systems make progress in spanning the semantic distance as compared to prior visualization tools. In particular, they all provide higher-level abstractions for visual encoding operations by automatically inferring appropriate definitions for scale functions and guides. Moreover, they all embed a ``live preview'' of the visualization that is automatically and immediately updated whenever the user manipulates an interface element. 

\leo{\textbf{What is Expressible}}\\
However, important differences exist in the semantics of the three visualization models. For example, in Charticulator, marks can only be instantiated via a glyph, which automatically produces one instance per data tuple. In contrast, marks in Lyra and Data Illustrator begin as standard shapes which can be moved or resized. This latter method allows for one-off annotation\,---\,a common technique in data-driven storytelling used to call a reader's attention to an area of interest. And, Data Illustrator goes a step further as its lazy data bind: if a data binding is removed, marks do not revert back to their previous, unbound appearance; a strategy that enables ``fuzzy'' layouts that approximate the original data values.

\leo{The underlying visualization model plays an important role in dictating what is expressible. For example, Data Illustrator does not currently have support to generate automatic graph layout, which is a given in Lyra. Although it is possible to add a graph layout module in Data Illustrator to constrain the position of nodes and edges. Is this mainly an issue of implementation? Should we focus on what is expressible using the visualization model or what is expressible in the actual system?}

Scale functions offer another point of comparison. While all three systems use scales to determine how data values are mapped to visual variables, and automatically infer their definitions, they vary the degree to which users are able to customize them. Charticulator allows users to customize scale domains and ranges, as well as toggle whether they are visualized by a guide. Data Illustrator offers this functionality in addition to the ability to merge scales such that a single scale function determines multiple encodings. This feature is useful for creating Gantt Charts, where the start and end times for tasks are enumerated as separate fields but must be plotted against the same scale. Lyra goes the furthest\,---\,by taking a grammar of graphics approach, it exposes scales as a first-class primitive that users can manually construct independent of data binding operations. This decoupling increases Lyra's expressive power, giving users fine-grained control over the scale domain, how scales are reused across the visualization, and how they are visualized by guides. For instance, users can create scales with hardcoded domains, a single scale that spans multiple distinct domains, or even add guides that visualize scales not used to determine any visual encodings\,---\,useful when emphasizing how values may exceed well-understood bounds.

Finally, all three systems exhibit an issue we dub \emph{schematic congruency}: authoring a visualization may require the backing dataset to be structured or formatted in a particular way that may not be clear to users a priori. In particular, all three systems expect datasets to have been cleaned externally and structured in a long (often referred to ``tidy'', and as opposed to wide) format. Data Illustrator and Charticulator do not provide any facility to transform the backing data, beyond sorting and calculating summary statistics such as the mean or median. Lyra, on the other hand, provides a palette of data transformations including operators to filter and aggregate the dataset, as well as derive new calculated fields\footnote{Vega's fold operator, used to transform a wide dataset into a long format, was added after Lyra's initial development; exposing it within Lyra would be a straightforward implementation effort.}. An additional set of layout transformations support ingesting non-tabular data (e.g., networks or geographies) but they impose their own set of structuring and formatting concerns that are invisible to the user. For example, the nodes and links of a network must be imported as two separate datasets, with each link described by properties named \texttt{source} and \texttt{target} exactly. 

Although supporting a rich set of data wrangling capabilities~\cite{kandel2011wrangler} is out of scope, how these systems should narrow schematic congruency remains an open question. As Lyra illustrates, it is not sufficient to simply extend the underlying visualization models to provide data transformation capabilities as expecting users to invoke and define them manually still presents a non-trivial semantic distance. Instead these systems must develop higher-level scaffolding that automatically infers or suggests appropriate transformations when necessary (analogous to their existing mechanisms for data binding which automatically infer definitions for scales and guides).

\leo{\textbf{Conciseness}}\\
\leo{The notion of efficiency might be relevant here (e.g. click count)}

\leo{\textbf{Gulf of Evaluation}}\\
\leo{In Data Illustrator, we couple the canvas and the Data Table Panel so that users can verify if the generated shapes have the right data scope. Selecting a visual item will show the data rows bound to that item. }\\


\leo{Todo: discuss rationales and tradeoffs}

%======================================================
\subsubsection{Articulatory Distance: How is it Expressed?}
%======================================================
Whereas semantic distance is concerned with the meanings of expressions in a user interface, articulatory distance describes how a user communicates this meaning or what form the expressions take. Like semantic distance, articulatory distance can occur on both the input and output ends of an interface as well. For example, consider zooming via a pinch gesture versus spinning the mouse wheel; the two interactions present a similar semantic distance, but pinching provides more articulatory directness. Similarly, on the output side, \arvind{TODO example}.

To analyze the articulatory distances the three systems present, we consider which actions can be performed on the visualization directly, and which must occur via property inspectors or configuration panels. For instance, marks in Lyra and Data Illustrator closely mimic the experience of drawing vector graphics as they can be repositioned or resized via mouse drags. Data Illustrator extends this metaphor to its repeat operator as well: users drag a collection's handles to increase or decrease the reptition. 

However, there are more salient differences in how the systems surface data binding. Lyra presents perhaps the shortest articulatory distance as users drag data fields and drop them into dropzones that overlay the selected mark on the visualization. Charticulator is one-step removed: users still drag fields, but the dropzones are displayed in a separate glyph panel. Data Illustrator, on the other hand, drives data binding through a dropdown menu in its property inspectors in order to reduce cursor travel. A Bubble Cursor effect~\cite{grossman2005bubble} might better balance these set of concerns, narrowing both the articulatory and cursor-travel distances\footnote{The latest development version of Lyra uses the Bubble Cursor effect to accelerate selection of the nearest dropzone. It is implemented via an invisible voronoi decomposition.}.

All three systems rely heavily on configuration panels, particularly for operations that do not have a clear direct manipulation analog. For example, data transformations in Lyra are created via button presses and manipulated via input widgets; Data Illustrator's partition operator is invoked with a button and dropdown menus in a dialog box are used to vary the stacking orientation; ...

- articulatory distance in terms of composition

Lyra's grammatical primitives, however, only offer compositional expressivity for basic cartesian layouts backed by tabular data. Though a ``reactive geometry''~\cite{satyanarayan2016reactive} makes it possible to anchor marks together, for more advanced layouts\,---\,such as stacking, pie charts, or treemaps\,---\,or data formats\,---\,including geographic, hierarchical, or network data\,---\,users must choose from a typology of data transformations. Data Illustrator's repeat and partition operators, on the other hand, offer a consistent mechanism for both basic and more advanced layouts but important implementation and conceptual limitations remain. For instance, partitioning a circle to produce a pie chart is conceptually well-defined but has not been implemented in the framework; however, how these operators extend to support geographic, hierarchical, or network data is an open conceptual question. Charticulator's system of constraints offers the most uniform underlying model but is exposed via 

- viscosity

==> xarchive/03b-learnability.tex <==
\subsection{Learnability}

Using Lyra, Data illustrator, or Charticulator requires a set of skills and a baseline visualization literacy that includes an understanding of concepts such as data binding. One of the required skills includes the ability to think computationally. Due to this requirement, how we assess the learnability of these systems will be largely dependent upon the skills and literacy of the people who use it and the those who we recruit as part of an evaluation process, in addition to the complexity of the content that people produce with these systems. Our informal observations after the deployment of these systems lead us to believe that people with programming knowledge are more prepared when it comes to using these systems. However, familiarity with the conventions set by existing design and visualization tools may interact with this learning process, helping in some cases and hindering in others, as these systems conform to different conventions to varying degrees. 

%======================================================
\subsubsection{Computational Thinking}
%======================================================
Our three systems each aspire to enable people to create charts without programming. However, to use these systems effectively and to realize its full potential, people benefit from being able to think computationally.

What makes Lyra intriguing from a learnability and computational thinking perspective is that Lyra is limited to the set of visualizations expressible in Vega~\cite{satyanarayan2016reactive}, and interactions in Lyra map to Vega statements. Lyra's production rules---the system of heuristics it uses to determine default values for scales, axes, and legends---have since subsumed by Vega-Lite~\cite{Satyanarayan2017VegaLite}. This prompts a question as to whether those who can already express themselves fluently in Vega or Vega-Lite are at an advantage when it comes to learning to use Lyra. However, Lyra's interface also diverges from computational thinking in other aspects. While Lyra was inspired by Victor's visualization authoring system~\cite{victor2013}, Victor's tool exposes the parameters of a programmatic control flow to the author; in contrast, Lyra hides this flow and instead allows for more direct manipulation of content.      
 
There is often a tradeoff between efficiency and learnability. As system designers and computational thinkers ourselves, the ability to achieve and demonstrate a high degree of efficiency in terms of creating a wide range of content is a recurring fixation, as reflected in the comparative click count comparison between systems reported in the Charticulator paper. However, Charticulator's emphasis on efficiency and reliance on computational thinking hinders its usability. For instance, it employs a simplified variant of regular expressions that enable people to format axis tick labels, such as controlling the number of decimal points or adding prefixes and postfixes for various numeric units. For people who are unfamiliar with the regular expressions, this is hardly learnable.

Overall, Charticulator largely employs a top-down approach, one that is ideal for people who know or are capable of intuiting what will happen when they perform actions like assigning a numerical data column with a particular domain to an axis spanning a physical range across the canvas, which presupposes the computational thinking required to understand data transformations. Another instance of computational thinking in Charticulator relates to its mapping of each data row to a glyph, where one glyph serves as a surrogate or prototype, representing all other glyphs in the chart. Therefore, while working with a glyph, people must be able to predict and understand the repercussions of their glyph design decisions on other glyphs as they work.



%======================================================
\subsubsection{Conformity}
%======================================================
One of the contributing factors behind a tool's learnability is the extent to which it conforms to or departs from the conventions established and perpetuated by the set of existing tools enjoying widespread use. For instance, aspects of Data Illustrator's interface can be traced to interface design conventions found in Tableau, Illustrator, Sketch, and XD (a vector design and wireframing application), and people with prior experience with these tools report having an easier time learning Data Illustrator. On the other hand, Charticulator notably departs from three notable conventions, thereby reducing its learnability. 

The first departure from convention pertains to an automatic creation of a legend, such as when binding a data column to the fill value of corresponding marks. In many tools (\eg Excel), a legend is automatically created when categorical data is used in a chart. Charticulator requires the designer to explicitly add a legend in one of two ways: adding a predefined legend layer to the chart after binding the column, or by specifying a custom legend with a new glyph in a separate plot segment. While these two options allow for considerable expressivity and flexibility in terms of the visual appearance and layout of the legend, these options incur a cost in terms of learnability. 

Another source of confusion is Charticulator's distinction between an axis and a legend; in many tools, both are created automatically, and thus the distinction does not enter into the mind of the designer. Consider the y-axis of a scatterplot (position) and the y-axis of a bar chart (length). To specify the former with Charticulator, one must bind a quantitative data column to the y-axis of a plot segment which will subsequently place a constraint on the vertical position of glyphs within that segment. To specify the latter, one must first bind a quantitative data column to the height of a rectangle mark in a glyph and subsequently toggle the appearance of a legend from that height binding. In both cases, the result is a chart element comprised of a vertical line accompanied by a set of evenly spaced ticks and labels, though one is considered to be an axis while the other is considered to be a legend. This discrepancy is an artifact of separating plot-level and glyph-level specification, which prioritizes expressivity over conformity.

A third violation of convention pertains to links between glyphs. Consider a line chart, where one might see each line as a single path mark. Charticulator offers no such mark. Instead, each line is a series of glyphs comprised of points whose positions are constrained by the plot segment's x and y axes, and the designer must explicitly toggle links to join these points using a devoted link specification interface. Similarly, Charticulator requires that each node in a node-link network diagram be specified as a glyph, and this glyph specification does not encompass the specification of the links between nodes, which must be explicitly toggled with the link interface. This separation of glyph and link is unique to Charticulator, and this uniqueness undoubtedly has a negative impact on its learnability.

While Charticulator departs from the conventions of many charting tools, the does not necessarily mean that its interaction paradigms are novel. For instance, its approach to specifying constraints is similar in spirit to the approach taken by the Android Studio IDE~\cite{AndroidConstraintLayout} for specifying constraints between mobile application user interface elements. However, we expect that the overlap between the population of mobile application developers using Android Studio and the population of chart designers to be small, and thus this interaction paradigm still defies the conventions of the chart designer community.

Despite attempts to leverage the conventions of existing tools, some new concepts cannot be communicated via these conventions. For instance, designers familiar with Adobe XD may be able to learn some aspects of Data Illustrator quickly as a result of common interface conventions. However, XD users with no prior experience in working with data still report difficulties understanding Data Illustrator's repeat and partition operators, as neither have a precedent in the XD interface.


==> xarchive/03c-reusability.tex <==
\subsection{Reusability}
Lyra: We get it from free via Vega, but this is the easy/cheap argument. Lyra hasn't done the necessary work to keep users at a high-level of abstraction when it comes to reuse. Instead, users will need to understand how to swap out data bindings with Vega’s runtime API, and if their visualizations break, they have no recourse except debugging the Vega specification (something unfamiliar).

Data Illustrator:  Does not currently support reproducing a visualization
Framework could potentially work for a homogenous dataset:
Lazy data-bindings, repeat/partition adjusts for the distribution of the data
No way to account for non-data driven changes, deletions of shapes, or bindings that were removed
Flexibility seems to be at odds with frameworks ability to support reproducibility



Charticulator: To enable people to design a wide range of chart designs that are reusable, Charticulator takes a constraint-based layout approach: because a chart design is specified through a set of constraints, the chart design can respond to a new canvas with a different size. One inherent limitation of Charticulator is thus it cannot handle popular algorithmic layouts such as treemap, force-directed layout, and wordle. In addition, it may not be feasible to represent a layout with semantics using a set of constraints (e.g., the standard waterfall chart that ends with zero). 

Users can import a Charticulator template, e.g. small multiples, require datasets to have the same columns 



Other subsequent additions included simple data manipulation capabilities, such as swapping out one dataset for another or the ability to perform simple aggregations; 

Charticulator and PowerBI's custom visual

Hanpuku, styling in dedicated graphics tools like Illustrator 



==> xarchive/03g-layout.tex <==
% !TEX root =  main.tex
%% =======================================================================
\subsubsection{Layout}
\label{sec:layout}
%% =======================================================================
\leo{Does it make sense to move this section before Section 3.2.5 ``Nesting and Small Multiples''? }\\
Lyra's grammatical primitives only offer compositional expressivity for basic cartesian layouts backed by tabular data. Though a ``reactive geometry''~\cite{satyanarayan2016reactive} makes it possible to anchor marks together, for more advanced layouts\,---\,such as stacking, pie charts, or treemaps\,---\,or data formats\,---\,including geographic, hierarchical, or network data\,---\,users must choose from a typology of data transformations. 

Data Illustrator's repeat and partition operators, on the other hand, offer a consistent mechanism for both basic and more advanced layouts but important implementation and conceptual limitations remain. For instance, partitioning a circle to produce a pie chart is conceptually well-defined but has not been implemented in the framework; however, how these operators extend to support geographic, hierarchical, or network data is an open conceptual question. 

Charticulator's system of constraints offers the most uniform underlying model for the layout and enables coordinate Systems such as polar and arbitrary curve coordinates, going beyond cartesian. 

\textbf{Manual Placement of Graphical Elements.}

- Charticulator + DI have them. 
  - Not data bound (vs. axes/legends).
- Lyra does not have guides.

% Lyra uses the term "guides" differently.
% Guides. Guides visualize scales, providing reference marks to aid interpretation. Axes visualize scales over a spatial domain, and include ticks, labels, and optional grid lines. Legends visualize scales for color, shape or size encodings. (p4)
% Visualizations in Lyra are compositions of visual elements: graphical marks and guides. (p5)


\textbf{Relative Layouts.}

- Charticulator: within, between glyphs.
- Lyra: connecting marks.

\textbf{Parametric Layouts vs. Algorithmic Layouts}

- DI: grid \& stacked.
%In general, we can apply the following types of layout to a collection generated by repeat: freeform (i.e. no layout), grid, stack, and packing. (p5)
%Both the grid and stack layouts have a coordinate space parameter consisting of two values: Cartesian and Polar. (p5)

- Charticulator: layout as constraints
%  - But UI/interactions are varied (e.g., drag-and-drop for data binding constraints, clicking checkbox for link constraints, etc.). %BL: a link itself is not a layout component
  - What can/cannot be expressed?
  - Does the user ever need to be aware that the system is expressing constraints? Does this ever leak?

- Lyra: advanced layouts supported by as button presses/property inspectors
  - Also often requires data to be in a custom format.
  - Some direct manipulation (eg laying out/pinning nodes, centering/scaling geo projections).
  - But inconsistent model so inconsistent interaction model: not a grammar of layout primitives but typology.


==> xarchive/04-discussion.tex <==
%% =====================================
\section{Discussion}
%% =====================================
